Learning to Regrasp by Learning to Place

In this paper, we explore whether a robot can learn to regrasp a diverse set of objects to achieve various desired grasp poses. Regrasping is needed whenever a robot's current grasp pose fails to perform desired manipulation tasks. Endowing robots with such an ability has applications in many domains such as manufacturing or domestic services. Yet, it is a challenging task due to the large diversity of geometry in everyday objects and the high dimensionality of the state and action space. In this paper, we propose a system for robots to take partial point clouds of an object and the supporting environment as inputs and output a sequence of pick-and-place operations to transform an initial object grasp pose to the desired object grasp poses. The key technique includes a neural stable placement predictor and a regrasp graph-based solution through leveraging and changing the surrounding environment. We introduce a new and challenging synthetic dataset for learning and evaluating the proposed approach. We demonstrate the effectiveness of our proposed system with both simulator and real-world experiments. More videos and visualization examples are available on our project webpage.

==> tex/exp.tex <==
In this work, we develop a learning framework for robots to learn to regrasp objects. Our experiments focus on evaluating the following questions: (1) How effective is our proposed learning-to-place approach compared to other baselines?  (2) Whether our proposed learning-to-regrasp pipeline can find good solutions to the object regrasping problem? (3) Whether the multi-task learning for contact point predictions we use in Sec.~\ref{sec:placeing} is useful or not? 
%\lin{ToDo: Updating the sentences grammar}

\vspace{-1mm}
\paragraph{Dataset.}
We construct a dataset containing 50 objects (i.e., spoon, fork, hammer, wrench, etc.) and 30 supporting items (i.e., mug, box, bowl). We then split these objects and supporting items into training and test sets. We generate 249 pairs from the training set of objects and supporting items, and 38 pairs from the test. For each pair of object-supporting item, the initial placement poses are generated by sampling different object poses with respect to the supporting item in PyBullet, and running a forward simulation to see if it remains stable. We collect the placement data for supporting items by randomly placing the supporting items with respect to the initial environment (i.e., the ground), and running the simulation to check whether the supporting items keep static. In total, we generate 1,050,884 poses for training items and 15,105 poses for testing items. We visualize the data in supplementary material.

\vspace{-1mm}
\paragraph{Settings.}
% \vspace{-2mm}
For evaluation, we set up the simulation environment in PyBullet~\cite{coumans2019} as visualized in Fig.\ref{fig:teaser}. A Franka arm mounted with a two fingered robotic-gripper is loaded in the simulation. We load the object at the predicted pose and check if there is collision and whether the object is stable. 

%\vspace{-1mm}
\subsection{Object Stable Placement}\label{sec:exp_placing}
%\vspace{-1mm}

We evaluate our proposed framework on learning stable placement poses in this subsection.
\begin{table}[ht]
\vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
method & \begin{tabular}[c]{@{}c@{}}bowl-\\ fork\end{tabular} & \begin{tabular}[c]{@{}c@{}}bowl-\\ spoon\end{tabular} & \begin{tabular}[c]{@{}c@{}}box-\\ hammer\end{tabular} & \begin{tabular}[c]{@{}c@{}}box-\\ wrench\end{tabular} & \begin{tabular}[c]{@{}c@{}}box-\\ spatula\end{tabular} & \begin{tabular}[c]{@{}c@{}}mug-\\ fork\end{tabular} & \begin{tabular}[c]{@{}c@{}}mug-\\ spoon\end{tabular} & \begin{tabular}[c]{@{}c@{}}mug-\\ corkscrew\end{tabular} & mean \\ \hline
Random & 0.000 & 0.001 & 0.109 & 0.039 & 0.000 & 0.000 & 0.000 & 0.012 & 0.020 \\ \hline
~\citet{jiang2012learning} & 0.037 & 0.080 & 0.201 & 0.113 & 0.047 & 0.018 & 0.125 & 0.092 & 0.089 \\ \hline
~\citet{jiang2012learning} + heuristic & 0.175 & 0.041 & 0.437 & 0.852 & 0.603 & 0.013 & 0.128 & 0.000 & 0.281 \\ \hline
Ours & \textbf{0.869} & \textbf{0.848} & \textbf{0.894} & \textbf{0.911} & \textbf{0.905} & \textbf{0.674} & \textbf{0.834} & \textbf{0.829} & \textbf{0.845} \\ \hline
\end{tabular}
}
\caption{Overall comparison of the stable placement accuracy. We report the accuracy of our method and different baseline methods for each category and the average accuracy over all the categories. Our method achieves the best performance.}
\label{tab:place_acc}
\vspace{-3mm}
\end{table}

\begin{wrapfigure}{r}{7cm}
\vspace{-4mm}
\centering
\includegraphics[width=\linewidth]{imgs/pose_gen_diversity.pdf}
\vspace{-2mm}
\caption{Point cloud visualization of sampled stable poses from our proposal network. Our proposal network can generate diverse stable placements of the candidate object (colored in green). We also mark the predicted stable scores.}\label{fig:pose_gen_diversity}
\vspace{-4mm}
\end{wrapfigure}


\vspace{-1mm}
\paragraph{Evaluation of Pose Proposal Network.} We first evaluate whether the pose proposal network can generate a reasonable distribution of the stable poses for placing the object over the supporting items, as a diversifying stable pose distribution is crucial for the success of finding desirable regrasping solutions. For each input pair, we draw 128 poses from the proposal network, and we transform the candidate object to the proposed stable poses, the qualitative results are presented in Fig.~\ref{fig:pose_gen_diversity}. Our visualization demonstrates that our proposed stable poses yield a diversifying object placement.     


\vspace{-1mm}
\paragraph{Evaluation of Pose Classifier.}
To evaluate how accurate the pose classifier is, we estimate the scores for the sampled and refined 128 poses using the pose classifier. We use a threshold of 0.8 to filter out all the unsure poses. For verifying the remaining poses, we run a forward simulation in PyBullet~\cite{coumans2019} to check whether the pose keep static, and the accuracy of stable placement for each category are reported in Table~\ref{tab:place_acc}.

We first adopt a baseline which is based on a random sampling strategy that draw the rotation from SO(3) uniformly, and translation is sampled from [$\pm 0.05$, $\pm 0.05$, $z$+0.02] in the supporting item's local frame, where $z$ is determined by the maximal height of each supporting item.

We also compare our approach with~\citet{jiang2012learning} in Table~\ref{tab:place_acc}. Followed their method, we randomly sample 128 poses in the local frame of the supporting environment, and filter out all the unstable poses using the learned classifier, the remaining ones are used for evaluating the accuracy in PyBullet~\cite{coumans2019} through running a forward simulation. The results suggest that even with random sampled poses, a simple classifier with hand-craft feature can improve the stable placement accuracy. We also test another baseline that adopt heuristic rules for pose sampling but with the same classifier from~\cite{jiang2012learning}. For this baseline, the object translation in XY dimension is sample in the radius of $0.9 * r$ and the translation in Z dimension is determined by $z+0.01$, both are in support's local frame, where $r$ and $z$ are the radius and maximal height of supporting item respectively. We additionally rotate the object to make the longest axis of the object to be parallel with the XY plane. While this baseline can achieve some reasonable results in some easier pairs that with a nearly flat surface (i.e., box-wrench, box-spatula), it perform worse with supporting items with complicated geometry (i.e., bowl, mug). The results demonstrate that a good pose proposal algorithm is also of great importance to the success of stable object placement. With carefully designed stable pose proposal network and stable pose classifier network, our framework achieves the best results over all the approaches.

% overall performances: 
% A1. easy case (object placement)---> Section 3.2: fixed supports: success rate , computation time, 
%   generator ---> initial poses ---> CEM ---> task checker 
%     (Proposed approach: mug is fixed and spoon is on the table, grasp the spoon and place it into the mug, grasp the handle)
%     (Random Placement approach, successfully grasp the spoon, random place, ? not sure whether you can regrasp it)
%   stable poses prediction success rate, regrasp success rate, computation time
    
% Fig 6. Qualitative Example (Regrasp whole Process)

% Ours:
% Baselines: 20, 40, 0
% Motion Planning: 100, 60, ~900

\vspace{-1mm}
\subsection{Object Regrasping Performance}
\vspace{-1mm}

\begin{wrapfigure}{r}{6cm}
\centering
\includegraphics[width=\linewidth]{imgs/vis.pdf}
\vspace{-4mm}
\caption{Visualization of two regrasping tasks. Top row: regrasp a hammer; Bottom row: regrasp a spoon.}\label{fig:more}
\vspace{-2mm}
\end{wrapfigure}
%\vspace{-2mm}

Leveraging the stable pose prediction model and object grasping model, we evaluate the regrasping performance of our proposed system. We randomly select multiple objects from our dataset when creating each initial manipulation scene. These objects are placed stably, except that the robot might grasp one object. In each scene, there is one regrasp query, which is a target grasp pose of one object, for our system to accomplish. In total, we have 30 scenes as the test set.

Our system generates the regrasp graph by predicting the stable poses of each object and checking whether there are edges connecting two nodes. The regrasp task is considered successful if our system finally finds the target regrasp poses. We report the average success rate among the test scenes. We adopt a baseline approach by replacing our object placement prediction model with the baseline method described in Sec.~\ref{sec:exp_placing} and keeping the same rest settings. Our proposed pipeline achieves 73.3\% success rate while the baseline does not have any successful case. More visualization results are available in the supplementary material. 
%\begin{figure*}[ht!]
%\centering
%\includegraphics[width=\linewidth]{imgs/example.png}
%\caption{examples.}\label{fig:sequence}
%\end{figure*}


\vspace{-1mm}
\subsection{Ablation Study: Does Multi-task Learning Help?}
\vspace{-1mm}
%We conduct an ablation study to validate the proposed multi-task learning framework.

%\vspace{-1mm}
%\paragraph{}

\begin{table}[]
\centering
\begin{tabular}{c|c c c c}
\hline
\hline
Task Combination & Contact Acc. & Contact Prec. & Stable Acc. & Stable Prec. \\ \hline
stable & N/A & N/A & 0.888 & 0.890  \\ \hline
stable + contact & 0.925 & 0.977 & \textbf{0.918} & 0.906 \\ \hline
stable + contact + offset (ours) & \textbf{0.945} & \textbf{0.981} & 0.912 & \textbf{0.910} \\ \hline
\end{tabular}
\vspace{1mm}
\caption{We report the performance of our model trained with different loss variants. Our multi-task joint learning strategy leverages the correlation between tasks to enhance the feature learning, which results in better generalization.}
\vspace{-4mm}
\label{tab: diff_loss}
\end{table}

To verify the usefulness of the multi-task joint learning framework, we adopt the same network architecture but with different combinations of task losses. The quantitative results on the test set are shown in Table~\ref{tab: diff_loss}. We use the accuracy and precision metrics to measure the performance of each model. While the model trained with only stable loss reaches a reasonable performance, adding auxiliary losses improves the stable precision from 0.906 to 0.910. Our experiments demonstrate that the contact prediction and contact offset regression are beneficial to the stable pose learning task. This is reasonable because a strong correlation between each subtask eases the joint learning process: 1) for all stable poses, the placed object must have contact points with the supporting environment, and 2) the offset from the support and the object should be consistent with each other. 

